Structural properties of non-spherical dark halos in Milky Way and Andromeda dwarf spheroidal galaxies

We investigate the non-spherical density structure of dark halos of the dwarf spheroidal (dSph) galaxies in the Milky Way and Andromeda galaxies based on revised axisymmetric mass models from our previous work. The models we adopt here fully take into account velocity anisotropy of tracer stars confined within a flattened dark halo. Applying our models to the available kinematic data of the 12 bright dSphs, we find that these galaxies associate with, in general, elongated dark halos, even considering the effect of this velocity anisotropy of stars. We also find that the best-fit parameters, especially for the shapes of dark halos and velocity anisotropy, are susceptible to both the availability of velocity data in the outer regions and the effect of the lack of sample stars in each spatial bin. Thus, to obtain more realistic limits on dark halo structures, we require photometric and kinematic data over much larger areas in the dSphs than previously explored. The results obtained from the currently available data suggest that the shapes of dark halos in the dSphs are more elongated than those of $\Lambda$CDM subhalos. This mismatch needs to be solved by theory including baryon components and the associated feedback to dark halos as well as by further observational limits in larger areas of dSphs. It is also found that more diffuse dark halos may have undergone consecutive star formation history, thereby implying that dark-halo structure plays an important role in star formation activity.

==> Reference.tex <==
\begin{thebibliography}{}
\bibitem[Agnello \& Evans(2012)]{AE2012} Agnello, A., \& Evans, N.~W.\ 2012, \apjl, 754, LL39 
\bibitem[Allgood et al.(2006)]{Alletal2006} Allgood, B., Flores, R.~A., Primack, J.~R., et al.\ 2006, \mnras, 367, 1781 
\bibitem[Amorisco et al.(2013)]{Amoetal2013} Amorisco, N.~C., Agnello, A., \& Evans, N.~W.\ 2013, \mnras, 429, L89 
\bibitem[Barber et al.(2015)]{Baretal2015} Barber, C., Starkenburg, E., Navarro, J.~F., \& McConnachie, A.~W.\ 2015, \mnras, 447, 1112 
\bibitem[Battaglia et al.(2011)]{Batetal2011} Battaglia, G., Tolstoy, E., Helmi, A., et al.\ 2011, \mnras, 411, 1013 
\bibitem[Binney \& Tremaine(2008)]{BT2008} Binney, J., \& Tremaine, S. 2008, Galactic Dynamics (2nd ed.; Princeton, NJ: Princeton Univ. Press)  
\bibitem[Boylan-Kolchin et al.(2011)]{Boyetal2011} Boylan-Kolchin, M., Bullock, J.~S., \& Kaplinghat, M.\ 2011, \mnras, 415, L40 
\bibitem[Boylan-Kolchin et al.(2012)]{Boyetal2012} Boylan-Kolchin, M., Bullock, J.~S., \& Kaplinghat, M.\ 2012, \mnras, 422, 1203 
\bibitem[Breddels \& Helmi(2013)]{BH2013} Breddels, M.~A., \& Helmi, A.\ 2013, \aap, 558, AA35 
\bibitem[Brook \& Di Cintio(2014)]{BD2014} Brook, C.~B., \& Di Cintio, A.\ 2015, \mnras, 450, 3920  
\bibitem[Brooks \& Zolotov(2014)]{BZ2014} Brooks, A.~M., \& Zolotov, A.\ 2014, \apj, 786, 87 
\bibitem[Bryan et al.(2013)]{Bryetal2013} Bryan, S.~E., Kay, S.~T., Duffy, A.~R., et al.\ 2013, \mnras, 429, 3316 
\bibitem[Burkert(1995)]{Bur1995} Burkert, A.\ 1995, \apjl, 447, L25 
\bibitem[Cappellari(2008)]{Cap2008} Cappellari, M.\ 2008, \mnras, 390, 71 
\bibitem[de Blok(2010)]{deB2010} de Blok, W.~J.~G.\ 2010, Advances in Astronomy, 2010, 789293 
\bibitem[de Blok et al.(2001)]{deBetal2001} de Blok, W.~J.~G., McGaugh, S.~S., Bosma, A., \& Rubin, V.~C.\ 2001, \apjl, 552, L23 
\bibitem[de Blok et al.(2008)]{deBetal2008} de Blok, W.~J.~G., Walter, F., Brinks, E., et al.\ 2008, \aj, 136, 2648 
\bibitem[Del Popolo \& Pace(2015)]{DP2015} Del Popolo, A., \& Pace, F.\ 2015, arXiv:1502.01947 
\bibitem[Di Cintio et al.(2014a)]{DiCetal2014a} Di Cintio, A., Brook, C.~B., Dutton, A.~A., et al.\ 2014, \mnras, 441, 2986 
\bibitem[Di Cintio et al.(2014b)]{DiCetal2014b} Di Cintio, A., Brook, C.~B., Macci{\`o}, A.~V., et al.\ 2014, \mnras, 437, 415 
\bibitem[Diemand et al.(2008)]{Dieetal2008} Diemand, J., Kuhlen, M., Madau, P., et al.\ 2008, \nat, 454, 735 
\bibitem[Donato et al.(2009)]{Donetal2009} Donato, F., Gentile, G., Salucci, P., et al.\ 2009, \mnras, 397, 1169 
\bibitem[Dutton et al.(2007)]{Dutetal2007} Dutton, A.~A., van den Bosch, F.~C., Dekel, A., \& Courteau, S.\ 2007, \apj, 654, 27 
\bibitem[Evans, An \& Walker(2009)]{Evaetal2009} Evans, N.~W., An, J., \& Walker, M.~G.\ 2009, \mnras, 393, L50 
\bibitem[Fukushige \& Makino(1997)]{FM1997} Fukushige, T., \& Makino, J.\ 1997, \apjl, 477, L9 
\bibitem[Garrison-Kimmel et al.(2013)]{Garetal2013} Garrison-Kimmel, S., Rocha, M., Boylan-Kolchin, M., Bullock, J.~S., \& Lally, J.\ 2013, \mnras, 433, 3539 
\bibitem[Gentile et al.(2005)]{Genetal2005} Gentile, G., Burkert, A., Salucci, P., Klein, U., \& Walter, F.\ 2005, \apjl, 634, L145 
\bibitem[Gentile et al.(2009)]{Genetal2009} Gentile, G., Famaey, B., Zhao, H., \& Salucci, P.\ 2009, \nat, 461, 627 
\bibitem[Gentile et al.(2007)]{Genetal2007} Gentile, G., Salucci, P., Klein, U., \& Granato, G.~L.\ 2007, \mnras, 375, 199 
\bibitem[Gilmore et al.(2007)]{Giletal2007} Gilmore, G., Wilkinson, M.~I., Wyse, R.~F.~G., et al.\ 2007, \apj, 663, 948 
\bibitem[Governato et al.(2010)]{Govetal2010} Governato, F., Brook, C., Mayer, L., et al.\ 2010, \nat, 463, 203 
\bibitem[Governato et al.(2012)]{Govetal2012} Governato, F., Zolotov, A., Pontzen, A., et al.\ 2012, \mnras, 422, 1231 
\bibitem[Hastings(1970)]{Has1970}Hastings, W. K. 1970, Biometrika, 57, 97
\bibitem[Hayashi \& Chiba(2012)]{HC2012} Hayashi, K., \& Chiba, M.\ 2012, \apj, 755, 145 
\bibitem[Hayashi \& Chiba(2015)]{HC2015} Hayashi, K., \& Chiba, M.\ 2015, \apjl, 803, L11
\bibitem[Hayashi et al.(2004)]{Hayetal2004} Hayashi, E., Navarro, J.~F., Power, C., et al.\ 2004, \mnras, 355, 794 
\bibitem[Hayashi et al.(2007)]{Hayetal2007} Hayashi, E., Navarro, J.~F., \& Springel, V.\ 2007, \mnras, 377, 50 
\bibitem[Ho~et al.(2012)]{Hoetal2012} Ho, N., Geha, M., Munoz, R.~R., et al.\ 2012, \apj, 758, 124 
\bibitem[Hoekstra et al.(2005)]{Hoeetal2005} Hoekstra, H., Hsieh, B.~C., Yee, H.~K.~C., Lin, H., \& Gladders, M.~D.\ 2005, \apj, 635, 73 
\bibitem[Irwin \& Hatzidimitriou(1995)]{IH1995} Irwin, M., \& Hatzidimitriou, D.\ 1995, \mnras, 277, 1354 
\bibitem[Ishiyama et al.(2013)]{Ishietal2013} Ishiyama, T., Rieder, S., Makino, J., et al.\ 2013, \apj, 767, 146 
\bibitem[Jardel \& Gebhardt(2013)]{JG2013} Jardel, J.~R., \& Gebhardt, K.\ 2013, \apjl, 775, LL30 
\bibitem[Jardel et al.(2013)]{Jaretal2013} Jardel, J.~R., Gebhardt, K., Fabricius, M.~H., Drory, N., \& Williams, M.~J.\ 2013, \apj, 763, 91 
\bibitem[Jing \& Suto(2000)]{JS2000} Jing, Y.~P., \& Suto, Y.\ 2000, \apjl, 529, L69 
\bibitem[Jing \& Suto(2002)]{JS2002} Jing, Y.~P., \& Suto, Y.\ 2002, \apj, 574, 538 
\bibitem[Kazantzidis et al.(2004)]{Kazetal2004} Kazantzidis, S., Kravtsov, A.~V., Zentner, A.~R., et al.\ 2004, \apjl, 611, L73 
\bibitem[Kleyna et al.(2002)]{Kleetal2002} Kleyna, J., Wilkinson, M.~I., Evans, N.~W., Gilmore, G., \& Frayn, C.\ 2002, \mnras, 330, 792 
\bibitem[Kirby et al.(2013)]{Kiretal2013} Kirby, E.~N., Cohen, J.~G., Guhathakurta, P., et al.\ 2013, \apj, 779, 102 
\bibitem[Koch et al.(2007a)]{Kocetal2007a} Koch, A., Grebel, E.~K., Kleyna, J.~T., et al.\ 2007, \aj, 133, 270 
\bibitem[Koch et al.(2007b)]{Kocetal2007b} Koch, A., Kleyna, J.~T., Wilkinson, M.~I., et al.\ 2007, \aj, 134, 566 
\bibitem[Kormendy \& Freeman(2004)]{KF2004} Kormendy, J., \& Freeman, K.~C.\ 2004, Dark Matter in Galaxies, 220, 377 
\bibitem[Kormendy \& Freeman(2014)]{KF2014} Kormendy, J., \& Freeman, K.~C.\ 2014, arXiv:1411.2170 
\bibitem[Kuhlen et al.(2007)]{Kuhetal2007} Kuhlen, M., Diemand, J., \& Madau, P.\ 2007, \apj, 671, 1135 
\bibitem[Madau et al.(2014)]{Madetal2014} Madau, P., Shen, S., \& Governato, F.\ 2014, \apjl, 789, LL17 
\bibitem[Martin et al.(2008)]{Maretal2008} Martin, N.~F., de Jong, J.~T.~A., \& Rix, H.-W.\ 2008, \apj, 684, 1075 
\bibitem[Mateo(1998)]{Mat1998} Mateo, M.~L.\ 1998, \araa, 36, 435 
\bibitem[Mateo et al.(2008)]{Matetal2008} Mateo, M., Olszewski, E.~W., \& Walker, M.~G.\ 2008, \apj, 675, 201 
\bibitem[McConnachie(2012)]{McC2012} McConnachie, A.~W.\ 2012, \aj, 144, 4 
\bibitem[McConnachie \& Irwin(2006)]{MI2006} McConnachie, A.~W., \& Irwin, M.~J.\ 2006, \mnras, 365, 1263 
\bibitem[Metropolis et al.(1953)]{Metetal1953} Metropolis, A. W., Rosenbluth, M. N., Teller, A. H., \& Teller, E. 1953, J. Chem. Phys., 21, 1087
\bibitem[Moore(1994)]{Moo1994} Moore, B.\ 1994, \nat, 370, 629 
\bibitem[Navarro et al.(1996)]{NFW1996} Navarro, J.~F., Frenk, C.~S., \& White, S.~D.~M.\ 1996, \apj, 462, 563 
\bibitem[Navarro et al.(1997)]{NFW1997} Navarro, J.~F., Frenk, C.~S., \& White, S.~D.~M.\ 1997, \apj, 490, 493 
\bibitem[Nipoti \& Binney(2015)]{NB2015} Nipoti, C., \& Binney, J.\ 2015, \mnras, 446, 1820 
\bibitem[Ogiya \& Burkert(2015)]{OB2015} Ogiya, G., \& Burkert, A.\ 2015, \mnras, 446, 2363 
\bibitem[Ogiya \& Mori(2014)]{OM2014} Ogiya, G., \& Mori, M.\ 2014, \apj, 793, 46 
\bibitem[O{\~n}orbe et al.(2015)]{Onoetal2015} O{\~n}orbe, J., Boylan-Kolchin, M., Bullock, J.~S., et al.\ 2015, arXiv:1502.02036 
\bibitem[Pe{\~n}arrubia et al.(2012)]{Penetal2012} Pe{\~n}arrubia, J., Pontzen, A., Walker, M.~G., \& Koposov, S.~E.\ 2012, \apjl, 759, L42 
\bibitem[Plummer(1911)]{Plu1911} Plummer, H.~C.\ 1911, \mnras, 71, 460 
\bibitem[Salucci et al.(2012)]{Saletal2012} Salucci, P., Wilkinson, M.~I., Walker, M.~G., et al.\ 2012, \mnras, 420, 2034 
\bibitem[Schneider et al.(2012)]{Schetal2012} Schneider, M.~D., Frenk, C.~S., \& Cole, S.\ 2012, \jcap, 5, 030 
\bibitem[Spano et al.(2008)]{Spaetal2008} Spano, M., Marcelin, M., Amram, P., et al.\ 2008, \mnras, 383, 297 
\bibitem[Strigari et al.(2010)]{Stretal2010} Strigari, L.~E., Frenk, C.~S., \& White, S.~D.~M.\ 2010, \mnras, 408, 2364 
\bibitem[Strigari et al.(2014)]{Stretal2014} Strigari, L.~E., Frenk, C.~S., \& White, S.~D.~M.\ 2014, arXiv:1406.6079 
\bibitem[Takada et al.(2014)]{Taketal2014} Takada, M., Ellis, R.~S., Chiba, M., et al.\ 2014, \pasj, 66, R1 
\bibitem[Tempel \& Tenjes(2006)]{TT2006} Tempel, E., \& Tenjes, P.\ 2006, \mnras, 371, 1269 
\bibitem[Teyssier et al.(2013)]{Teyetal2013} Teyssier, R., Pontzen, A., Dubois, Y., \& Read, J.~I.\ 2013, \mnras, 429, 3068 
\bibitem[Tollerud et al.(2012)]{Toletal2012} Tollerud, E.~J., Beaton, R.~L., Geha, M.~C., et al.\ 2012, \apj, 752, 45 
\bibitem[van der Marel et al.(1994)]{vanetal1994} van der Marel, R.~P., Evans, N.~W., Rix, H.-W., White, S.~D.~M., \& de Zeeuw, T.\ 1994, \mnras, 271, 99 
\bibitem[Vera-Ciro et al.(2014)]{Veretal2014} Vera-Ciro, C.~A., Sales, L.~V., Helmi, A., \& Navarro, J.~F.\ 2014, \mnras, 439, 2863 
\bibitem[Walker et al.(2009a)]{Waletal2009a} Walker, M.~G., Mateo, M., \& Olszewski, E.~W.\ 2009, \aj, 137, 3100 
\bibitem[Walker et al.(2009b)]{Waletal2009b} Walker, M.~G., Mateo, M., Olszewski, E.~W., Sen, B., \& Woodroofe, M.\ 2009, \aj, 137, 3109 
\bibitem[Walker et al.(2009c)]{Waletal2009c} Walker, M.~G., Mateo, M., Olszewski, E.~W., et al.\ 2009, \apj, 704, 1274 
\bibitem[Walker \& Pe{\~n}arrubia(2011)]{WP2011} Walker, M.~G., \& Pe{\~n}arrubia, J.\ 2011, \apj, 742, 20 
\bibitem[Weisz et al.(2014)]{Weietal2014} Weisz, D.~R., Dolphin, A.~E., Skillman, E.~D., et al.\ 2014, \apj, 789, 147 
\bibitem[Weisz et al.(2015)]{Weietal2015} Weisz, D.~R., Dolphin, A.~E., Skillman, E.~D., et al.\ 2015, \apj, 804, 136 
\bibitem[Wolf et al.(2010)]{Woletal2010} Wolf, J., Martinez, G.~D., Bullock, J.~S., et al.\ 2010, \mnras, 406, 1220 
\end{thebibliography}


==> tab1.tex <==
%%% Table 1 %%%
\begin{deluxetable*}{ccccccccc}
\label{tb:tab1}
\tablecolumns{9}
\tablewidth{7.0in}
\tablecaption{The observational dataset for MW and M31 dSph satellites}
\tablehead{
Object & No. of stars & $M_{\ast}$ & $M_V$  & $D_{\odot}$ & $r_{\rm half}$ &  $q^{\prime}$  & ${\tau}_{0.7}$\tablenotemark{a}  &   Ref.\tablenotemark{b} \\
          &                             & ($10^6M_{\odot}$)  &  & (kpc) & (pc) & (axial ratio) & (Gyr) & }
\startdata
MW dSphs & & & & & & & &\\
Carina     & 776   & $0.38$     & $-9.1 \pm 0.5 $       &$106\pm6$     & $241\pm 23$       & $0.67\pm0.05$   & $4.5$    & 1,3,7\\
Fornax    & 2523 & $20.0$     & $-13.4 \pm 0.3 $     & $147\pm12$  & $668\pm 34$       & $0.70\pm0.01$   &  $4.6$   & 1,3,7\\
Sculptor  & 1360 & $2.3  $     & $-11.1 \pm0.5 $       & $86\pm6$     & $260\pm 39$       & $0.68\pm0.03$   &  $12.7$ & 1,3,7 \\
Sextans  & 445   & $0.44$     & $-9.3 \pm0.5 $       & $86\pm4$     & $682\pm 117$      & $0.65\pm0.05$   &  No data & 1,3,7 \\
Draco     & 185   & $0.29$     & $-8.8 \pm0.3 $        & $76\pm6$     & $196\pm 12$        & $0.69\pm0.02$   &  $11.5$  & 2,7 \\
Leo~I      & 328   & $5.5 $     & $-12.0 \pm0.3 $      & $254\pm15$ & $246\pm 19$        & $0.79\pm0.03$   &  $2.7$   & 2,3,7 \\
Leo~II     & 200   & $0.74 $     & $-9.8 \pm0.3 $    & $233\pm14$  & $151\pm 17$        & $0.87\pm0.05$   &  $6.8$  & 1,7 \\
M31 dSphs & & & & & & & &\\
And~I       & 51    & $3.9  $    & $-11.7 \pm0.1 $     &$745\pm24$    & $670\pm 30$        & $0.78\pm0.04$   & $7.6$  & 5,6,7\\
And~II      & 488  & $7.6  $    & $-12.4 \pm0.2 $  & $652\pm18$    & $1230\pm20$       & $0.90\pm0.02$   & $6.2$  & 4,6,7\\
And~III     & 62    & $0.83$    & $-10.0 \pm0.3 $ & $748\pm24$    & $400\pm 30$       & $0.48\pm0.02$   & $8.8$  & 5,6,7 \\
And~V     & 85     & $0.39$     & $-9.1 \pm0.2 $    & $773\pm28$    & $350\pm 20$       & $0.82\pm0.05$   & $10.0$ & 5,6,7 \\
And~VII   & 136   & $9.5  $  & $-12.6 \pm0.3 $    & $762\pm35$    & $770\pm 20$       & $0.87\pm0.04$   & $12.8$ & 5,6,7
\enddata
\tablenotetext{a}{This value is the lookback time at achieving $70\%$ of current stellar mass of dSphs, and is estimated by available data taken from~\citet{Weietal2014}.}
\tablenotetext{b}{References: (1)~\citet{IH1995}; (2)~\citet{Maretal2008}; (3)~\citet{Waletal2009c}; (4)~\citet{Hoetal2012};~(5)~\citet{Toletal2012}; (6)~\citet{MI2006}; (7)~\citet{McC2012}} 
\end{deluxetable*}

==> tab2.tex <==
%%% Table 2 %%%
\begin{deluxetable*}{cccccccc}
\label{tb:tab2}
\tablecolumns{8}
\tablewidth{7.0in}
\tablecaption{Results of MCMC analysis for twelve dSph galaxies.}
\tablehead{
Galaxy       &      $Q$                  & $b_{\rm halo}$[pc]                & $\rho_0$ $[$M$_{\odot}$ pc$^{-3}$]         &  $\beta_z$         & $\alpha$            &$i$ [deg]            &    $L_{\rm prolate}/L_{\rm oblate}$}
\startdata
MW dSphs  &&&&&&&\\
Carina        &   $0.33\pm0.02$    &  $709.7^{+40.6}_{-44.3}$      & $0.107\pm0.006$   &  $-0.05\pm0.06$                 &  $-0.09^{+0.09}_{-0.05}$                &  $87.1^{+2.9}_{-9.1}$      &      $0.0056$ \\ 
Fornax       &   $0.38\pm0.03$    &  $991.1^{+27.0}_{-21.4}$       & $0.086\pm0.003$   &  $-0.17^{+0.16}_{-0.07}$       &  $0.00_{-0.04}$                              &  $90.0_{-10.6}$             &     $0.28$\\ 
Sculptor    &   $0.45\pm0.03$    &  $637.7^{+32.6}_{-26.0}$      & $0.168\pm0.008$   &  $-0.03^{+0.06}_{-0.04}$     &  $0.00_{-0.09}$                              &  $87.8^{+2.2}_{-9.1}$     &      $0.000015$\\ 
Sextans     &   $0.53\pm0.06$    &  $1126.7^{+93.5}_{-74.5}$    & $0.028\pm0.008$   &  $ 0.23^{+0.12}_{-0.18}$       &  $0.00_{-0.10}$                              &  $89.8^{+0.2}_{-12.5}$   &      $0.54$\\ 
Draco        &    $0.40\pm0.05$    &  $590.2^{+46.5}_{-43.9}$     & $0.153\pm0.021$   &   $0.31^{+0.08}_{-0.13}$       &  $-0.86^{+0.11}_{-0.11}$                  &  $75.6^{+14.4}_{-8.8}$   &     $0.21$\\ 
Leo~I        &    $0.86\pm0.10$    &  $581.8^{+33.3}_{-26.1}$      & $0.037\pm0.005$   &  $0.09\pm0.14$                   &  $-1.40^{+0.06}_{-0.08}$                 &  $70.5^{+19.5}_{-7.5}$   &      $0.68$\\ 
Leo~II      &    $0.91\pm0.16$    &  $281.8^{+35.3}_{-30.6}$      & $0.195\pm0.031$    &  $-0.62^{+0.56}_{-1.8}$       &  $0.00_{-0.11}$                                &  $88.8^{+0.2}_{-34.3}$   &     $0.91$\\ 
M31 dSphs  &&&&&&&\\
And~I       &    $2.41^{+0.49}_{-0.39}$     &  $811.3^{+118.1}_{-112.7}$           & $0.037\pm0.009$   &  $0.79^{+0.03}_{-0.05}$     &  $-0.39^{+0.39}_{-0.29}$       &  $90.0_{-34.8}$            &   $0.16$\\
And~II     &    $0.32\pm0.06$               &  $1112.2^{+54.8}_{-55.2}$           & $0.005\pm0.004$    &  $-0.13^{+0.31}_{-0.87}$    &  $-1.03\pm0.09$                     &  $85.2^{+4.8}_{-25.4}$    & $35.1$\\
And~III   &    $0.16\pm0.04$                  &  $796.9^{+90.5}_{-96.8}$           & $0.043\pm0.01$      &  $\leq -0.21$                      &  $-1.43^{+0.14}_{-0.23}$         &  $70.8^{+8.6}_{-3.3}$     &  $0.53$\\
And~V       &    $4.75^{+4.54}_{-1.71}$     &  $369.9^{+35.6}_{-37.2}$           & $0.039\pm0.007$   &  $\leq   0.13$                      &  $-1.33^{+0.21}_{-0.12}$         &  $78.2^{+11.8}_{-14.3}$     &  $0.35$\\
And~VII   &    $0.47\pm0.03$               &  $700.3^{+53.1}_{-44.2}$           & $0.041\pm0.008$    &  $0.57^{+0.09}_{-0.13}$    &  $-1.34^{+0.20}_{-0.16}$         &  $81.2^{+8.8}_{-15.7}$   & $10.2$
\enddata
\end{deluxetable*}

==> tab3.tex <==
%%% Table 3 %%%
\begin{deluxetable*}{cccccccc}
\label{tb:tab3}
\tablecolumns{8}
\tablewidth{5.8in}
\tablecaption{Comparison of best-fit parameters estimated from full data sample with those estimated from data only within half-light radius.}
\tablehead{Object  &  Data  &  $Q$  &  $b_{\rm halo}$[pc]  &  $\rho_0$ $[$M$_{\odot}$ pc$^{-3}$]  &  $\beta_z$  & $\alpha$  &  $i$ [deg]}
\startdata
Fornax   &   Data within $r_{\rm half}$   &   $0.83\pm0.04$   &   $708.5^{+23.1}_{-16.7}$   &   $0.101\pm0.004$   &   $0.40\pm0.03$   &  $-0.14\pm0.06$   &  $89.5^{+0.5}_{-10.6}$ \\
              &   Full data                                &   $0.38\pm0.03$   &   $991.1^{+27.0}_{-21.4}$   &   $0.086\pm0.003$   &   $-0.17^{+0.16}_{-0.07}$   &  $0.00_{-0.04}$   &  $90.0_{-10.6}$ \\
&&&&&&&\\
Sculptor &   Data within $r_{\rm half}$   &   $0.73^{+0.07}_{-0.04}$   &   $450.7^{+31.3}_{-17.7}$   &  $0.241\pm0.014$   &   $0.48\pm0.05$   &  $-0.02^{+0.02}_{-0.06}$   &  $89.5^{+0.5}_{-10.6}$ \\
              &   Full data                                &   $0.45\pm0.03$    &  $637.7^{+32.6}_{-26.0}$  &  $0.168\pm0.008$    &   $-0.03^{+0.06}_{-0.04}$  &  $0.00_{-0.09}$   &  $87.8^{+2.2}_{-9.1}$
\enddata 
\end{deluxetable*}


==> tab4.tex <==
%%% Table 4 %%%
\begin{deluxetable*}{cccccccc}
\label{tb:tab4}
\tablecolumns{8}
\tablewidth{6.7in}
\tablecaption{Best-fit parameters for considering photometric measurement errors}
\tablehead{Object  &  Measurement error  &$Q$  &  $b_{\rm halo}$[pc]  &  $\rho_0$ $[$M$_{\odot}$ pc$^{-3}$]  &  $\beta_z$  & $\alpha$  &  $i$ [deg]}
\startdata
Fornax   &   {\bf Half light radius}     &&&&&&\\    
              & Upper limit   &   $0.39\pm0.02$   &   $941.3^{+26.2}_{-17.8}$   &   $0.087\pm0.005$   &   $-0.13\pm0.08$   &  $0.00_{-0.04}$   &  $90.0_{-10.5}$ \\
             &  Lower limit  &   $0.40\pm0.02$   &   $924.7^{+23.5}_{-20.2}$   &   $0.094\pm0.006$   &   $-0.10\pm0.09$   &  $-0.04\pm0.04$  &  $88.6^{+1.4}_{-8.5}$ \\

              &   {\bf Projected  axial ratio}  &&&&&&\\
              & Upper limit   &   $0.40\pm0.02$   &   $887.9^{+28.1}_{-14.9}$   &   $0.095\pm0.004$   &   $-0.16^{+0.10}_{-0.06}$   &  $-0.01^{+0.01}_{-0.03}$   &  $90.0_{-12.1}$ \\
              &  Lower limit   &  $0.37\pm0.02$   &   $1013.9^{+22.8}_{-25.7}$ &   $0.088\pm0.004$   &   $-0.09^{+0.06}_{-0.13}$   &  $0.00_{-0.05}$   &  $90.0_{-10.8}$ \\
&&&&&&&\\
Sextans &  {\bf  Half light radius}  &&&&&&\\
              & Upper limit   &   $0.69\pm0.08$   &   $1110.6^{+95.1}_{-70.1}$   &   $0.024\pm0.002$   &   $0.37\pm0.11$   &  $0.00_{-0.09}$   &  $90.0_{-12.0}$ \\
              &  Lower limit  &   $0.36\pm0.05$   &   $1410.1^{+161.1}_{-101.1}$ &   $0.026\pm0.003$   &   $\leq 0.16$   &  $-0.10^{+0.08}_{-0.06}$   &  $89.7^{+0.3}_{-12.1}$ \\
              &  {\bf Projected  axial ratio}  &&&&&&\\
              & Upper limit   &   $0.78\pm0.08$   &   $896.7^{+60.7}_{-52.7}$   &   $0.030\pm0.003$   &   $0.38^{+0.07}_{-0.10}$   &  $-0.10^{+0.10}_{-0.08}$   &  $89.8^{+0.2}_{-14.8}$ \\
             & Lower limit    &   $0.48\pm0.06$   &   $1047.7^{+74.6}_{-68.1}$   &   $0.033\pm0.003$   &   $0.29^{+0.11}_{-0.13}$   &  $-0.02^{+0.02}_{-0.08}$   &  $89.5^{+0.5}_{-11.1}$ \\
&&&&&&&\\
And~II   &  {\bf Distance}  &&&&&&\\
               & Upper limit   &   $0.51\pm0.03$   &   $2886.1^{+165.8}_{-110.4}$   &   $0.0085\pm0.002$   &   $0.17\pm0.08$   &  $-0.01^{+0.01}_{-0.07}$   &  $89.8^{+0.2}_{-12.1}$ \\
               &  Lower limit  &   $0.53\pm0.03$   &   $2818.4^{+147.6}_{-150.5}$   &   $0.0093\pm0.002$   &   $0.28^{+0.04}_{-0.07}$   &  $0.00_{-0.042}$   &  $89.7^{+0.3}_{-12.5}$ \\
And~VII &  {\bf Distance}  &&&&&&\\
               & Upper limit   &   $1.87^{+0.45}_{-0.30}$   &   $411.5^{+33.1}_{-26.2}$   &   $0.078\pm0.012$   &   $-0.03^{+0.35}_{-0.54}$   &  $-0.76^{+0.27}_{-0.31}$   &  $70.0^{+20.0}_{-14.1}$ \\
              & Lower limit    &   $1.61^{+0.38}_{-0.27}$    &   $480.5^{+37.5}_{-32.7}$ &   $0.068\pm0.01$     &   $-0.05^{+0.33}_{-0.76}$   &  $-0.61^{+0.24}_{-0.30}$   &  $70.1^{+19.9}_{-14.6}$
\enddata 
\end{deluxetable*}
